RNR-Nav: A Real-World Visual Navigation System Using Renderable Neural Radiance Maps

We propose a novel visual localization and navigation framework for real-world environments directly integrating observed visual information into the bird-eye-view map. While the renderable neural radiance map (RNR-Map) shows considerable promise in simulated settings, its deployment in real-world scenarios poses undiscovered challenges. RNR-Map utilizes projections of multiple vectors into a single latent code, resulting in information loss under suboptimal conditions. To address such issues, our enhanced RNR-Map for real-world robots, RNR-Map++, incorporates strategies to mitigate information loss, such as a weighted map and positional encoding. For robust real-time localization, we integrate a particle filter into the correlation-based localization framework using RNRMap++ without a rendering procedure. Consequently, we establish a real-world robot system for visual navigation utilizing RNR-Map++, which we call "RNR-Nav." Experimental results demonstrate that the proposed methods significantly enhance rendering quality and localization robustness compared to previous approaches. In real-world navigation tasks, RNR-Nav achieves a success rate of 84.4%, marking a 68.8% enhancement over the methods of the original RNR-Map paper.

==> figures/system.tex <==
\centering
\begin{tabular}{cc}
\begin{tabular}{c} \includegraphics[width=0.55\linewidth]{figures/system_new} \end{tabular} &
\begin{tabular}{c} \includegraphics[width=0.35\linewidth]{figures/robot2} \end{tabular} \\
\begin{tabular}{@{\hspace{-0.1cm}}c@{\hspace{-0.5cm}}} (a) \textbf{RNR-Nav Framework} \end{tabular} &
\begin{tabular}{@{\hspace{-0.1cm}}c@{\hspace{-0.5cm}}} (b) \textbf{Robot System} \end{tabular}\\
\end{tabular}

==> tables/recon_result_backup.tex <==
\begin{tabular}{ccc|cccccc|cccccc}

\toprule
\multicolumn{3}{c|}{} & \multicolumn{6}{c|}{\textbf{Online}} & \multicolumn{6}{c}{\textbf{Offline}\textbf} \\
\multicolumn{3}{c|}{} & \multicolumn{3}{c}{\textbf{Seen}} & \multicolumn{3}{c|}{\textbf{Full}\textbf} & \multicolumn{3}{c}{\textbf{Seen}} & \multicolumn{3}{c}{\textbf{Full}\textbf} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}
Weight & PE & Mip & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$  \\
\midrule
\xmark & \xmark & \xmark & 16.365 & 0.466 & 0.612 & 16.263 & 0.463 & 0.613 & 16.318 & 0.465 & 0.613 & 16.315 & 0.466 & 0.613 \\
\checkmark & \xmark & \xmark & 16.389 & 0.468 & 0.609 & 16.287 & 0.466 & 0.610 & 16.351 & 0.468 & 0.611 & 16.607 & 0.470 & 0.610 \\
\checkmark & \checkmark & \xmark & \textbf{19.348} & \textbf{0.574} & 0.536 & \textbf{19.128} & \textbf{0.569} & 0.538 & \textbf{19.164} & \textbf{0.571} & 0.536 & \textbf{19.156} & \textbf{0.571} & 0.536 \\
\midrule
\checkmark & \checkmark & \checkmark & 19.283 & 0.573 & \textbf{0.531} & 19.061 & \textbf{0.569} & \textbf{0.534} & 19.113 & \textbf{0.571} & \textbf{0.533} & 19.106 & \textbf{0.571} & \textbf{0.532} \\
\bottomrule

\end{tabular}
